Comparing Generic and Community-Situated Crowdsourcing for Data Validation in the Context of Recovery from Substance Use Disorders

Targeting the right group of workers for crowdsourcing often achieves better quality results. One unique example of targeted crowdsourcing is seeking community-situated workers whose familiarity with the background and the norms of a particular group can help produce better outcome or accuracy. These community-situated crowd workers can be recruited in different ways from generic online crowdsourcing platforms or from online recovery communities. We evaluate three different approaches to recruit generic and community-situated crowd in terms of the time and the cost of recruitment, and the accuracy of task completion. We consider the context of Alcoholics Anonymous (AA), the largest peer support group for recovering alcoholics, and the task of identifying and validating AA meeting information. We discuss the benefits and trade-offs of recruiting paid vs. unpaid community-situated workers and provide implications for future research in the recovery context and relevant domains of HCI, and for design of crowdsourcing ICT systems.

==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

==> author_tenure_distribution.tex <==
\begin{figure}
\centering
\includegraphics{figures/author_tenure_distribution.pdf}
\caption{Distribution of author tenure---the time between first and last journal update written by that author---for all 572,309 author users. The 161,799 (28.3\%) authors with only a single update (and thus 0 tenure) are not shown. Median author tenure is 83 days (mean 311 days). We observe an approximately bimodal lognormal distribution of author tenure, fitting a two-component log-normal GMM in an approach inspired by Halfaker et al. \cite{halfaker_user_2015}.
Using the intersection of the two components, we include only authors with a tenure > 1 day.
}
\label{fig:author_tenure_distribution}
\end{figure}

==> table.tex <==
\begin{center}
\begin{table}\textwidth
\begin{tabular}{|p{.88in}|c|c|c|c|c|c|}
\hline
& \multicolumn{2}{c|}{\bfseries Page validation} & \multicolumn{2}{c|}{\bfseries Meeting validation} & \multicolumn{2}{c|}{\bfseries Meeting identification} \\
\cline{2-7}
  & Before filtering & Final \# & Before filtering & Final \# & Before filtering & Final \# \\
\hline
Generic: MTurk & A & A & A & A & A & A\\
\hline
Community-situated: MTurk & B & B & B & B & B & B\\
\hline
Community-situated: ITR & C & C & C & C &C & C\\
\hline
\end{tabular}
\label{tab:numparticipants}
\caption{Number of total participants for each task}
\end{table}
\end{center}



\begin{center}
\begin{figure}[t]
\begin{tabular}{ c c }
\begin{subfigure}{0.45\textwidth}
      \includegraphics[width=\textwidth]{figures/ITRhomebanner.png}
      \caption{}
    \end{subfigure}    &
    
    \begin{subfigure}{0.45\textwidth}
      \includegraphics[width=\textwidth]{figures/ITRnewsletter.png}
      \caption{}
    \end{subfigure} 
\end{tabular}
 \caption{The paid banner advertisement on the ITR website: (a) homepage, (b) newsletter}
 \label{fig:ads}
\end{figure}
\end{center}







\newcolumntype{P}[1]{>{\centering\arraybackslash}p{#1}}
\begin{center}
\begin{table}[t]
\begin{tabular}{|P{0.28\textwidth} | P{0.3\textwidth} | P{0.32\textwidth}|}
    \hline
      & Worker cost only (average cost per worker) & Total worker cost including platform cost (average cost per worker)\\
     \hline
     Generic: MTurk & \$2175 (\$2.5) & \$2718.75 (\$3.125)\\
     \hline
     Community-situated: MTurk & $\$1125 (\$2.5) + \$19.80 (\$0.03) = \$1099.80$ & \$1431 (\$3.18) \\
     \hline
     Community-situated: ITR & \$0 (\$0) & \$6000 (\$13.33)  \\
     \hline
\end{tabular}
\caption{Worker costs for generic and community-situated crowdsourcing. Worker cost is the portion of the total cost paid to only the workers for their task completion, and not to the platform}
\label{tab:workerandplatformcost}
\end{table}
\end{center}

==> temp.tex <==
\begin{comment}


Authors on CB may be either patients (P) or caregivers (CG).  This role may be contextual: multi-site authors may take a caregiver role on one site and a patient role on a second, an author may use a single site for recounting both a patient and caregiver perspective, or account sharing may result in updates published by the same author that are written by both a patient and one or more of that patient's caregivers.  To tease apart these factors, we classify authorship at the journal update level, aggregating to the author- and site-level based on the classification of updates published by that author or on that site.  

We trained a machine learning classifier to predict the author role of 15,850,052 updates%
\footnote{19,137,078 total updates exist in the dataset, but we remove spam updates, machine-generated updates, and updates less than 50 characters.} that were authored on valid sites.
%(82.8\%)
We acquired author role annotations from two previous CB studies, in addition to annotations acquired while doing exploratory data analysis and conducting active sampling on earlier iterations of the classifier.  To ensure the reliability of role identification, we computed an inter-rater reliability measure, as is appropriate for our quantitative goals and applying an existing codebook/taxonomy of author roles~\cite{mcdonald_reliability_2019}. Two of the authors independently annotated 429 updates, resulting in a Cohen's $\kappa$ of 0.829, which we determined to indicate sufficient reliability for this study~\cite{landis_measurement_1977}.  After annotation, we used as ground truth data 6,932 human-annotated updates from 305 sites\footnote{Note: 44 ground-truth updates (0.63\%) were assigned ambiguous or mixed labels that were reassigned to CG for training, reflecting a predominant interest in patients: the classifier is trained to predict if updates are patient-authored or not.}.

As the annotated data are not i.i.d.\ due to the use of data sampled from a different subset of CB data \cite{levonian_bridging_2020}, we train with balanced classes by randomly downsampling the P-labeled updates, an approach we found to outperform other training regimes e.g. training with all ground truth data.  We used hold-one-out cross validation to evaluate the performance of the model and to compare algorithmic approaches.  As a shared site/author could leak information about the held-out data and give an overly optimistic view of classifier performance, we hold out at the site level rather than holding out individual updates. We used a linear SVM classifier on TFIDF-transformed unigram and bigram features, a common and effective approach to binary text classification tasks~\cite{wang_baselines_2012}.
Accuracy was 95.08\% and micro-averaged F1 score was 0.95.  
P updates ($n=5938$, precision = 0.99, recall = 0.95, F1 = 0.97) were classified correctly at a greater rate than CG updates ($n=994$, precision = 0.77, recall = 0.93, F1 = 0.84).  

We computed the proportion of patient-authored updates on valid sites using a random sample of 5000 unlabeled journal updates.  We used the 305 models trained during hold-one-out cross validation in order to compute standard error as an estimate of the variability of this proportion.  The model predicted that 24.84\% (s.e. 0.03\%) of unlabeled journal updates were patient-authored.  As the label distribution in the training data is different from the label distribution over the target updates, we need to correct for this distribution shift as it will bias the estimate towards the balanced training distribution.  We use Black Box Shift Estimation (BBSE) \cite{lipton_detecting_2018} to quantify the shift in distribution and produce a revised estimate, finding that 22.06\% (s.e. 0.11\%) of unlabeled journal updates were patient-authored when BBSE is used.

To estimate the proportion of P/CG authors and sites, we aggregate update-level classifications.  We identify both sites and authors as either P, CG, or Mixed.  Through manual investigation of 30 sites, we identified a variety of usage patterns, including a high frequency of sites with at least one update from the non-majority author role.  To assess the general patterns in author role and to allow for error introduced by the classifier, we use a consistent set of thresholds: CG sites/authors have less than one third of their updates classified as patient-authored, Mixed sites/authors have between one third and two thirds of their updates classified as patient-authored, and P updates have more than two thirds of their updates classified as patient-authored.  Such thresholds are reasonable because the resulting labels encode the general perspective of an author, along with the associated differences in responsibilities and communication behavior. Further, these permissive thresholds keep cascading errors to a minimum.
In the cross-validated ground truth data, sites were classified at least two-thirds correctly 87.87\% of the time.  In the case of sites with all-P or all-CG updates (which should be unambiguously classified as P and CG respectively), this suggests a site-level error rate of at most 12.12\%. Qualitatively, we did not notice any clear errors among P- and CG-labeled authors, but in a sample of 30 sites and associated authors, Mixed-labeled authors were harder to interpret.  A taxonomy with further theoretical justification could be used in future work, but the approach used here has sufficient validity for comparing the behavior of P and CG authors.
% Feels a little unjustified here. Wondering if we need to do some randomly-sampled annotations in order to produce a user-level error rate estimate (and/or a better site-level error rate estimate).

Applying the definitions above, we find: For authors, 74.77\% are classified as CG, 17.74\% as P, and 7.49\% as Mixed.  
For sites, 74.09\% are classified as CG, 17.42\% as P, and 8.48\% as Mixed.  
Mixed-author accounts may indicate either a single author embodying multiple roles or multiple authors sharing the same account credentials.  Such account sharing generally occurs for convenience in the case of a trusted relationship between the patient and the caregiver \cite{jacobs_caring_2016}.  This account sharing is potentially problematic for analyses treating interactions between accounts as interactions between two humans, but particularly so if an account is shared by both a patient and a caregiver. 
Thus, we classify an author account as Shared if, on any site, between one third and two thirds of that author's updates are classified as patient-authored. 
Using this conservative definition, we find only 7.46\% of accounts are Shared%
\footnote{A more permissive definition labels author accounts as Shared if on any site that author has published both a P and a CG update. While this definition---which labels 53.4\% of accounts as Shared--- likely captures primarily classifier noise, it can be treated as an upper bound on author account sharing.}.
As expected, author account sharing is closely linked to the Mixed classification: 95.9\% of Mixed authors are Shared.  
Due to this high correlation, in subsequent modeling we include as an author feature only the Mixed author role and not an indicator of account sharing.

\section{Author interactions \& network structure}  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Inter-author interaction types \& analysis period}

\begin{table}[]
\begin{tabular}{@{}lrrrr@{}}
\toprule
           & All      & From valid authors & Non-self-interactions & Unique interactions\\ \midrule
Guestbooks & 82,980,359 & 5,864,304            & 5,212,720  & 687,432 \\
Amps       & 63,314,738 & 3,536,819            & 3,037,844  & 267,283 \\
Comments   & 31,052,715 & 1,094,435            & 881,781 & 197,188 \\ 
\textbf{Total} & \textbf{177,347,812} & \textbf{10,495,558} & \textbf{9,132,345} & \textbf{914,602} \\ \bottomrule
\end{tabular}%
\caption{Interaction counts by type. This study considers only interactions from valid authors to valid sites. Self-interactions are interactions on sites where the interacting author has published an update. Unique interactions is the count of unique non-self author/site pairs of each type; the total unique is computed irrespective of types and is thus lower than the sum of unique interaction pairs by type.}
\label{tab:int_type_counts}
\end{table}

\input{interaction_counts_over_time}

To study the interactions between authors, we construct a network from the log data in the CB dataset.  No direct interaction between users is possible on CaringBridge; instead, users interact with sites.  \textit{Guestbooks} are text posts left by a CB user on a site\footnote{Guestbooks were renamed ``Well Wishes'' by CB, but we exclusively use the older name.}.  \textit{Comments} are text posts left by a CB user on a specific journal update on a site.  \textit{Amps} are binary ``likes'' left by a CB user on a specific journal update on a site.  In this paper, we consider only interactions from valid authors to valid sites, with counts as shown in Table \ref{tab:int_type_counts}.  

Figure \ref{fig:interaction_counts_over_time} shows the number of each interaction type on CB over time.  Note the introduction of amps and comments as features on CB.  In order to avoid irregularities related to the introduction of new interaction types and to analyze a more established version of the network, many analyses will focus on the state of the network from January 1, 2014 to June 1, 2016, which we refer to as the \textit{analysis period}.  When models are fit to the interactions data, Jan 2014 -- Jan 2016 (80\% of the analysis period) is treated as training and inference data, and Jan 2016 -- Jun 2016 (the remaining 20\%) is treated as the test data and target for prediction.

Each interaction is associated with a unique identifier for the user and the site, as well as a timestamp.  Amps lack timestamp information, so we assume that amps occur at the publication time of the associated journal update.  
To assess whether this assumption is reasonable, we examine the moment when the amps feature was introduced, reasoning that amps on journal updates published before the amps feature launched indicate a lag time between the update publication and the amp interaction. 
Only 0.32\% of amps occur before the launch of the amps feature, and comparing updates published the week before the launch to the updates published in the week after, only 23.1\% of amps are recorded pre-launch.
This analysis suggests that the majority of amps are given in the week the journal update was published.

\subsection{Constructing the author interaction network}

We can construct a two-mode network \cite{latapy_basic_2008} containing both site and author nodes by drawing edges between authors and sites if any interaction exists between that author and that site.  As shown in Table \ref{tab:int_type_counts}, if we exclude interactions from authors to sites on which they have published any update as \textit{self-interactions} (12.99\% of all interactions), such a network has 915K edges.  Constructing a directed one-mode network containing only author nodes requires assumptions about the intended user target of any author's interaction with a site. We assume that, when an interaction occurs, that interaction links the interacting author to all authors who have previously written an update on that site.  
In addition, based on qualitative analysis of CB sites, we find that many guestbooks and comments are directed to both the caregiver authors of a site and the patient themselves, who may not yet be a CB user or have published an update on the site for which they are the subject.
Thus, we also draw an edge between the interacting author and any authors on the site who \textit{will} publish a patient-classified update. Such patient-specific edges are relatively uncommon; of the 1,144,492 edges in the one-mode author interaction network, 4.9\% of them are drawn to patient authors who had not yet published at the time of the interaction.  Using these assumptions, 9.1M author$\to$site interactions becomes 14.8M author$\to$author interactions, of which 1.1M are unique and thus form the edges within the network.

%We use the term \textit{initiations} to refer to the first interaction between any two authors.  The initiation network and the interaction network have the same set of edges.  
%The next sections will explore initiations in detail. 
%To reason about the growth of the initiation 

\subsection{Interaction network structure}

TODO Waiting on some refined visualizations and analysis from Drew. But this is mostly all I plan to say in this subsection. I might add a table with descriptive statistics about the network at the end of the analysis period: I would report diameter, max indegree and outdegree (along with distribution histograms, perhaps?), largest SCC size, largest WCC size, and \# of SC and WC components.

We offer a brief description of the overall structure of the network formed by author interactions on CaringBridge in order to understand the context in which interactions are occurring.
As the network is directed, components of connected authors can be identified as strongly connected---meaning a set of authors all reachable following the directed edges in the network---or weakly connected---meaning a set of authors all reachable following edges in any direction in the network.  The simplest strongly-connected component (SCC) is two authors who have interacted with each other. The simplest weakly-connected component (WCC) is two authors where one author has interacted with the second, but that interaction has not been reciprocated.
Figure XX shows the proportion of active authors in the largest weakly-connected component over time.  
CaringBridge seems to resemble other online health groups, in that it is dominated by a single large WCC \cite{rains_coping_2018,introne_sociotechnical_2016}. We observe a lack of isolated subnetworks, echoing \cite{urbanoski_investigating_2017}; at the end of the analysis period, there are only X strongly-connected components, with the second largest connecting only X authors.

%Urbanoski found that removing health educators does not substantially change the overall structure of the network i.e. strong core and periphery \cite{urbanoski_investigating_2017}, is that true for us and patients/caregivers?  Could say something simple about centrality: i.e. caregivers are more central, etc., or show the ``network over time'' visualizations but only including CG nodes or P nodes.  (This actually does seem interesting to me: does the Patient-only network look broadly the same?  Or does its growth and network look different?)

We do not observe a ``gelling point'' \cite{mcglohon_weighted_2008} in which many previously-unconnected components merge, accelerating the growth in size of the largest WCC.  This lack of gelling point may be related to the left-censored nature of our network data; interactions before 2005 are not present in our data.  Due to the importance of early members to the ultimate structure of Internet communities \cite{carron-arthur_community_2016}, this missing data may contain the history needed to observe the initial formation of the largest WCC.

\subsection{Other interactions}

In the author interaction network, we include only guestbooks, amps, and comments, as described above.  However, we omit three types of interaction that may behave differently than the included interaction types: (1) author visits to other sites, (2) comments on other comments, and (3) explicit or text-based links to other sites in journal updates. 
First, we omit visits because our visit data is incomplete and can be only tenuously linked to specific authors at specific times and is invisible to the receiving site's authors.  Second, we omit comments left in response to guestbooks and update comments as the feature is relatively recent and minimally used.  Third, inter-site HTML links can be published in the text of journal updates.
%can be either explicit HTML links or mentioning a CaringBridge URL slug in a journal update.  
To assess the impact of excluding such text-based inter-site links on the validity of the resulting network, we conducted a high-precision analysis of existing inter-site links.
Direct hyperlinks were extracted from the 19M journal updates. 101,923 valid links to CB sites were identified, of which 32.2\% (32,767) were determined to be self-links i.e. they linked to the site on which the update was authored.
%Links were extracted by matching the URL slug ``https://www.caringbridge.com'' or the HTML tag ``href'' associated with the URL slug.
Of the remaining 69,156 inter-site link interactions, 100\% were found to be redundant with existing interactions recorded via the other interaction types between the update author and the linked site.
Thus, we conclude that the three interaction types used provide a sufficiently detailed view of the inter-author interaction network.
%Updates analyzed: 19137078
%Links extracted: 3837736, of which 101923 are valid. 
%Self interactions: 32767 (non-self: 69156)

The CB interaction network reflects only interactions occurring publicly on CB, but additional interaction occurs off of CB.  Interaction can occur in response to CB updates but via a medium other than CB \cite{rains_social_2011}, but we study only on-site interaction.

% TODO This is also where we would say something about non-author interactions on CB. Is this necessary?

\section{Author initiations}  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

To address RQ1, we build quantitative models to describe the initiations between authors.  We first provide high-level context for initiations at the network-level.  Second, we differentiate authors who initiate with any others from authors who never initiate.  Third, we of authors who do initiate, we explore when they initiate with others. Fourth, we model with whom authors initiate as a function of both the initiator and the receiver.  

``Does a path exist between authors?'' variable comes from \cite{yan_network_2015}.

There is limited demographic and geographic homophily in OHCs \cite{yan_network_2015}; while we observe few demographic variables and no geographic info, per prior work we expect the effects to be relatively less important than other experiential similarity factors.

\subsection{In what network context? Initiation types}

\input{initiation_types_timeline}

Initiations between authors can be classified by the network position of the initiator and the receiver.
We adapt the definitions from Gallagher et al. to our context~\cite{gallagher_reclaiming_2019}:
(1) \textit{Joining Component} is an initiation connecting an unconnected author to an existing weakly-connected component with at least two existing connected authors.
(2) \textit{Bridging Component} is an initiation connecting two weakly-connected components, merging them.
(3) \textit{Joining Isolates} is an initiation that connects two previously unconnected authors (i.e. two ``isolates'').
(4) \textit{Intra Component} is an initiation between two authors who were already in the same weakly-connected component. By definition, all reciprocations are Intra Component initiations.

Figure \ref{fig:initiation_types_timeline} shows the proportion of each type of initiation during the growth of the CB network.  The balance of the four types is quite consistent within the analysis period.  
In the analysis period, Bridging Component and Joining Isolates combined make up only 3.62\% of the initiations.  The vast majority of initiations are between authors in the largest weakly-connected component and other members of the LWCC or previously unconnected authors.  
10.79\% of initiations in the analysis period are reciprocal, which is 13.91\% of the Intra Component initiations.
Of the Joining Component initiations, 41.30\% are initiated by the unconnected author and not someone in the component. In the analysis period, that proportion drops to 24.08\%.  Taken together, this suggests that vast majority of the initiations are occurring within the largest WCC (only 3.5\% of Intra Component initiations involved components other than the largest).
Thus, understanding the more local context and specific author features that lead to initiating is critical, as is addressed in subsequent analyses.

% Raw counts:
%     Intra Component   155996     77.54%
%   Joining Component    37905     18.84%
% Bridging Components     3761      1.87%
%    Joining Isolates     3526      1.75%

%\subsection{Modeling features}

%In order to address subsequent questions about the functioning of initiations on CB, we build mathematical models from features that capture the roles, demographics, and behaviors of the authors. This section describes the features used... (Or something like this)


\subsection{Who? Initiating authors}

\input{is_initiator_logreg_table}

Which authors initiate during their time on CB, and which do not? To understand the importance of factors such as author role, we fit a logistic regression model predicting if an author has initiated or not.  To avoid bias in the model from right-censoring---some authors will initiate but only after the end of our data collection period---we actually predict an outcome of initiating within 1 year of first authorship.  Similarly, we include a feature describing if an author was interacted with by another author in the first year.  Only 11.7\% of authors initiate more than 1 year from their first update.  Only 2.4\% of authors are interacted with more than 1 year from their first update.  Models with non-bounded outcomes and predictors produced similar results.

\subsubsection{Features}
In addition to author role, we included update count---the number of updates published by that author on CB---as well as update frequency---the ratio of that count to the author's tenure, rescaled to updates per month---as indicators of author activity level. Binary indicators for the mixed-site and multi-site author designations are included as potential confounders.  

We also include a self-reported categorical feature for health condition.
When CB users create a site, they have the option to self-report a broad health condition category such as Cancer or Injury.  While only 59.1\% of valid sites self-report a health condition and such single-label categorization may be overly reductive \cite{li_condition_2018}, this self-reported data can still serve to inform us about differences in inter-author communication behavior based on the health condition under question.  This data also enables us to confirm expected patterns in increased interaction between users who share a health condition~\cite{thoits_stress_2010,rains_social_2016}.
We assign health conditions (HCs) to authors based on the reported health condition of the sites they've authored, using the designation `None' when no condition is reported. 
For the 3.1\% of authors with multiple sites that report different health conditions, we assign the first non-None/Condition Unknown health condition reported.
Only 446 authors have sites with multiple non-None/Condition Unknown health conditions.  
Author HC assignment counts by condition are shown in Appendix Table \ref{app:tab:health_condition_category_counts}.
%Total users: 362345
%Users with multiple sites: 20057
%Users with multiple sites that have multiple conditions associated with them: 11102
%Users with multiple sites and multiple non-None/Condition Unknown conditions: 446

\subsubsection{Results}

Table \ref{tab:init_logreg_full_comparison} shows three models predicting author initiation within their first year on CB. In a model not shown, we observed a strong impact of being interacted with on initiation behavior; being interacted with is associated with a 182\% increase in the odds of initiating. Thus, we fit two additional models, splitting the data by whether they had been interacted with, shown as models (2) and (3) in Table \ref{tab:init_logreg_full_comparison}.
When an author is not interacted with, being a P rather than a CG author is associated with a 30\% decrease in the odds of initiation.  When an author is initiated with, being a P is associated with a 21\% increase in the odds of initiation.  
This disparity suggested a potential interaction effect between being interacted with and author role.  Table \ref{tab:init_logreg_interaction_term} shows this interaction, which shows that P authors are much more likely to be initiators after being interacted with compared to CG, although both P and CG are more likely to initiate after being interacted with.

We observe differences in initiation probability by health condition. For example, compared to reporting no health condition, an author self-reporting Cancer is associated with an 11\% increase in the odds of initiating.  However, we caution against over-interpretation of the less-common health conditions categories such as Congenital/Immune Disorder.
Activity level and authorship configuration have small affects on probability of initiation. In a separate model predicting if an author is interacted with, rather than if they initiate, these effects are more relevant, as could be expected. Each additional update published is associated with a 1\% increase in the odds of being interacted with, and being a mixed-site author is associated with a 123\% increase in the odds of being interacted with (versus a 15\% increase in the odds of initiating).

\subsection{When? Initiation timing}

\input{init_timing_response_plot}

\input{init_timing_effects_plot}

\begin{table}
\begin{center}
\begin{tabular}{lrrrrrr}
Feature      &  Coef.  & Std.Err. &    t     & P$>$$|$t$|$ &  [0.025 &  0.975]  \\
\hline

Intercept                                                  & -6.2153 &   0.1216 & -51.1311 &      0.0000 & -6.4536 & -5.9771  \\
AR = Mixed                             & -0.6622 &   0.4220 &  -1.5691 &      0.1166 & -1.4894 &  0.1650  \\
AR = P                                 & -0.8250 &   0.2607 &  -3.1643 &      0.0016 & -1.3361 & -0.3140  \\
Total Active Time (months)                                &  0.9348 &   0.0030 & 309.5406 &      0.0000 &  0.9289 &  0.9408  \\
Total Active Time 
: AR = Mixed &  0.0049 &   0.0099 &   0.4952 &      0.6205 & -0.0145 &  0.0243  \\
Total Active Time : AR = P     & -0.0195 &   0.0072 &  -2.7212 &      0.0065 & -0.0335 & -0.0055  \\
\hline
\end{tabular}
\end{center}
\caption{Placeholder for interaction model shown in effects plot.  Other stats to report:
R squared is 0.86.
F-stat 25300 ($p < 0.001$).
Model df 5.
Observations 20687.
Log-likelihood -75495.}
\label{tab:init_timing_author_type_interaction}
\end{table}

Given that an author is going to initiate, when is their first initiation likely to occur?  Among the valid users, the first initiation occurs pre-authorship 20.82\% of the time, i.e. before that author published their first journal update.
Echoing the results from the previous section, only 3.72\% of initiating authors do so post-authorship but before receiving an interaction, with the majority of initiating authors (75.46\%) initiating after authoring their first update and receiving an interaction.
We treat these the pre-authorship initiator and the post-authorship initiator separately, fitting linear regression models to predict the number of months between first authorship and initiation.  Figure \ref{fig:init_timing_response_plot} shows the distribution of this interval.  

\subsection{Features}
In the case of post-authorship, we compute ...

\subsection{Results}

Table \ref{tab:init_timing_author_type_interaction}

Figure \ref{fig:init_timing_effects_plot}

An ANOVA test confirms the significance of the interaction term at the 99\% significance level (F=4.07, p<0.01).

Appendix Table \ref{tab:init_timing_full_models}

\subsection{With whom? Initiation target}

We now turn to the question of who an author initiates with given that they are initiating with someone.
We model initiations between authors as discrete choices.
Following Overgoor et al., we fit multinomial logistic models to evaluate the relative importance of various factors associated with authors \cite{overgoor_choosing_2019}.
Multinomial logistic models are (description coming from Saumik).  
We use R to fit all models \cite{mlogit_package}.
(Here's how to interpret the coefficients of the model, approximately.)

\subsubsection{Conditional multinomial logit models}

Unedited text from Saumik.

 Social networks can be described as dynamic directed graph, where each node in the graph is a unique user and each edge is a connection initiated between a user and another user. The formation of the entire network is therefore the set of directed connections between users over time. In this paper, we are building from the methods described in Overgoor et al, where each new edge is considered a discrete choice made by the initiating user. The goal of this framework is to understand the features which can explain the choices of nodes selected for connection.

In order to model edge formation as discrete choices, we use the Conditional Multinomial Logit Model. Conditional logit models work particularly well for modelling choices in a graph for two reasons. First, they can be used to represent common network formation mechanisms, like preferential attachment, node fitness, and latent space models. Second, conditional logit models allow the combination of multiple features and mechanisms into one model, and let us learn their relative importance in the combined model.

When learning a conditional logit model on a specific decision, we train by considering both the actual decision made by the node, and the set of possible decisions that the node could have taken instead. For example, if the node has chose to connect with one node, out of 100,000 possible nodes, then this one edge actually generates 1 positve training sample, and 99,999 negative training samples. However large graphs can make training slow. We can improve the runtime of the conditional logit model by employing Negative Sampling. Instead of training on each negative sample, we randomly select a much smaller subset of these samples to train on.

Once enough positive and negative samples are collected, we can then train the conditional logit models. Depending on which features we are interested in, we can create multiple models using subsets of the features. For each trained model, a set of coefficients are calculated for each feature, as well as a standard error for the estimate. The magnitude of the coeffieicnts is dependent on the domain of each individual feature, so it is impossible to compare these magnitudes across features with different magnitudes. Instead, we can interpret the feature importance by looking at the sign. A positive sign means the presence of the feature is positively correlated with node selection, while a negative sign means a negative correlation with node selection. We can use the standard error values to make claims about the statistical significance of each feature. Finally, we can run the conditional logit models on a test set to determine the overall model accuracy.

\subsubsection{Features}

When comparing if two authors share the same health condition, we construct a dummy variable that is 1 when the two authors are assigned the same non-None health condition and 0 otherwise.


\subsubsection{Results}

We find that a shared user role (P/CG) between CB users increases the likelihood that they will form a connection. This echoes findings in other online contexts that users tend to communicate with others in similar health-related roles \cite{xu_twitter_2015}.

Using the same approach described in \cite{pan_you_2017} (elaborate), we find that support giving is highly reciprocal; received replies is highly correlated with sent replies.

In the next section, we investigate reciprocation behavior more specifically and under what conditions reciprocated initiations become connections with repeated interactions (relationships).

\subsubsection{Geographic analysis}

One important confounder in studying initiations on CB is the geographic proximity of CB authors.  Geographic proximity may indicate existing offline social ties and post-diagnosis connections made in-person rather than on CaringBridge.  While a fine-grained investigation of geographic effects on the relationship between the CB interactions network and the social networks of P/CG is out-of-scope for this work, we generate a rough proxy for geographic proximity by assigning US states to authors based on the IP addresses of their journal updates and guestbooks%
\footnote{Our data do not capture IP addresses for amps or comments.}.

We use the Maxmind GeoLite2 City database (from Aug 13, 2019) to do IP geolocation lookups\footnote{\url{https://dev.maxmind.com/geoip/geoip2/geolite2/}}. We refer to journal updates and guestbooks that are assigned identifiable geographic coordinates as \emph{geo-identifiable posts}. 
93\% of CB authors' geo-identifiable posts are entirely based in the United States.  Among these authors, we attempt to assign US states as our proxy for geographic proximity.  We avoid the direct use of latitude/longitude estimates to reduce the bias introduced through the use of IP geolocation \cite{poese_ip_2011}.

A US state is assigned to an author if that author has at least 10 geo-identifiable posts and among those posts the most-frequently-occurring state holds a plurality with at least a 20\% margin above the second most frequent state, with the intent of creating a high-precision, low-recall state assignment.  32.7\% (118,534) of authors are assigned states using this procedure.  As a face validity check, the most frequent state assignments are Minnesota (6.3\%; CaringBridge was launched in Minnesota), California (2.8\%; the most populous US state), and Texas (2.8\%; the second most populous US state).  This author sample is more active, more likely to have IP addresses that can be geo-identified, more likely to have a plurality of their updates in a single US state, and more likely to initiate with other authors (2.41 vs 2.26 mean initiations, $p<0.001$) than the average CB author.  

In the analysis period, initiations between state-assigned authors account for only 4.5\% (7,007) of the total initiations.  49.5\% of these initiations were between two authors that share the same US state assignment, a percentage significantly above chance.  Fitting a full multinomial logit model that includes a dummy variable when the initiating author and the candidate author share a state assignment confirms the importance of this feature: sharing a state assignment increases the odds of initiating with an author, holding other variables fixed, by 1422 times.  (The model details and full comparison is shown in Appendix \ref{app:geo_analysis}, Table \ref{app:tab:geo_full_model_comparison}.) Fitting a model with only that feature results in a test accuracy (on 668 initiations in the test period) of 27.8\%.  This analysis suggests the importance of geographic co-location, although given the biased nature of the proxy used it is hard to reason about the magnitude of this effect relative to the other contextual factors.  At a minimum, geographic co-location is an important predictor of initiation for at least some subset of authors.  

\subsection{Qualitative: What is the relationship between initiator and receiver?}\label{sec:qual_relationship_type_annotation}

Unedited text from G in this section. TODO Revise this into a slightly conciser analysis of relationship between the two people.

To develop an understanding between the authors of the various journal updates and those who interacted with them, the contents of the comments and guestbook entries on the updates were examined. Each comment or guestbook entry chosen for this purpose was authored by a user who already had their own CaringBridge site at the time, or will have started one in the future. After choosing the 100 comments and guestbook entries each made by these users, they were analyzed manually to determine two things: the commenter’s relationship with the author of the update, and whether the commenter’s connection with the author of the update was post the diagnosis of the patient being written about in the blog. It was also the case that each entry so chosen was made by a user who had never before interacted with the author of the blog post where the entry was being made, so the commenting user was determined to be an initiator. The relationship between the initiator and the author was given one value from the following list: Self, Friend, Parent, Coworker, Online Acquaintance, Fellow Patient, Family Member, Son/Daughter, Spouse, Caregiver, Unknown. The possibility of the connection being post-diagnosis was either True, Maybe or False. 

While considering initiations by virtue of comments on journal updates, it was observed that the nature of the initiator’s relationship with the author of the journal update could not be definitively determined in 69\% of the cases. This number indicates that a lot of comments were left by users who simply chanced upon the site in some way, and chose to leave good wishes or a show of support for the patient. For guestbook initiations, this percentage remained similar, with 63\% of the guestbook entries were made by initiators with an unclear relationship to the patient. 
	
It is worth noting, however, that a lot of these connections were labeled as Unknown because it could not be determined with certainty whether the initiator was a Friend, Family Member or an Online Acquaintance.  

This lack of clarity in determining the connection made sense when examining the post-diagnosis connections. The data revealed that 7\% of comment initiations and 13\% of the guestbook initiations were definitely post-diagnosis, while 27\% of comment initiations and 29\% of the guestbook initiations were definitely pre-diagnosis. In trying to identify these, qualitative markers in the text proved to be decisive. When initiators signed off with “Uncle” or similar familial ties, or spoke of some shared memories from the past, the connections were clearly pre-diagnosis. Similarly, if initiators mentioned meeting the patient in treatment facilities, rehab centers, support groups or other facilities that the two met at, then the connection was determined to be post-diagnosis. Furthermore, when the initiator was either a fellow patient receiving treatment at the same care facility as the author, or a patient who had/has a similar condition and is offering support, the connection was also determined to be post-diagnosis. Only in the absence of such clear markers was a connection labeled as Maybe post-diagnosis. 

\section{Dyadic relationships}  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

In this section, we investigate reciprocation behavior more specifically and under what conditions reciprocated initiations become connections with repeated interactions (relationships).

Still not sure what to say here, since our results are more spotty here.

One good result: Patients are more likely to reciprocate than CGs, CGs are more likely to reciprocate with patients than other caregivers, and Ps are MUCH more likely to reciprocate with other patients.  Story is: reciprocation is uncommon (5\% among CGs), but much more common when initiations involve patients! (19\% among Ps!) See Table \ref{tab:recip_role_probs}.
Controlling for the role of the initiator and the receiver, the initiator and the receiver sharing an author role is associated with a 55.7\% increase in the odds of a reciprocation.

\input{recip_role_probs}

%\section{Outcomes of condition-motivated connections on authors}

%We follow previous research in using continued online communication with others as a proxy for perceiving and receiving support from those others \cite{rains_social_2016}.

%Rains and Wright identify five potential limitations for participation in online support communities that may increase the stress of users. The following five conditions may increase patient or caregiver stress: (a) exposure to the difficulties experienced by others, (b) seeing others improve and making unfavorable social comparisons, (c) becoming overly focused on one's illness, (d) lack of immediate feedback, (e) limited or negative feedback.

%We expect differential effects of network connections based in part on individual difference factors such as personality or preference for weak-tie support \cite{rains_social_2016,wright_measure_2010}.  In light of these differential effects, we conduct a log analysis on patients and caregivers with high-ITE and low-ITE, adapting the motivations and perspective of trace ethnography \cite{geiger_operationalizing_2017} to identify key factors not included as observable covariates in our matching model and to validate the approach.


\section{Discussion}  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Implications for design}

Recommendation.
Connection recommendation should take network characteristics into account \cite{yan_network_2015}.
There have been calls to connect caregiver family members of cancer patients with others in a similar position \cite{sanden_cancer_2019}.
Other sources that motivate a focus on recommendation: \cite{cohen_social_2004,oleary_design_2017,eschler_im_2017,newman_its_2011,chen_make_2009}

Important to understand the context in which people are forming connections before attempting to change the way connections are formed, as support interventions often do not work as intended (meaning minimal effect) \cite{lakey_social_1996,eysenbach_health_2004}.

The observed appropriative use of CB for inter-author communication may indicate a lack of appropriate channel for this communication in the readily-available communication technologies already in use \cite{sleeper_sharing_2016}.

\section{Limitations}  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

The interaction network is a partial view of the true social network. And the population that engages at all will differ from patients and caregivers who don't initiate according to a variety of demographic and psychosocial factors \cite{han_lurking_2014,rains_social_2016}.

We may be particularly interested in serendipity, but isolating it is hard.

Single study platform.

Confounding can easily wreck us \cite{jackson_social_2010}, and we can't differentiate homophily effects from contagion effects \cite{shalizi_homophily_2011}.

Tie strength not accounted for \cite{burke_growing_2014,burke_relationship_2016}

We don't look at outcomes, especially outcomes of patients' efforts to connect with others online, which are critical and an important area for further research \cite{rains_coping_2018}.
While explorations of web-based social support have found correlations between social support and lower stress, experimental interventions have not always found a decrease in stress, even as received support has increased for treated participants \cite{hill_influence_2006}.
\end{comment}
